Non-linearities in the Lyman-$\alpha$ forest and in its cross-correlation with dark matter halos

Three-dimensional correlations of the Lyman-$\alpha$ (Ly$\alpha$) forest and cross correlations between the Ly$\alpha$ forest and quasars have been measured on large scales, allowing a precise measurement of the baryon acoustic oscillation (BAO) feature at redshifts $z>2$. These 3D correlations are often modelled using linear perturbation theory, but full-shape analyses to extract cosmological information beyond BAO will require more realistic models capable of describing non-linearities present at smaller scales. We present a measurement of the Ly$\alpha$ forest flux power spectrum from large hydrodynamic simulations -- the Sherwood simulations -- and compare it to different models describing the small-scale deviations from linear theory. We confirm that the model presented in Arinyo-i-Prats et al. (2015) fits the measured 3D power up to $k=10\, h\rm{Mpc^{-1}}$ with an accuracy better than 5%, and show that the same model can also describe the 1D correlations with similar precision. We also present, for the first time, an equivalent study for the cross-power spectrum of halos with the Ly$\alpha$ forest, and we discuss different challenges we face when modelling the cross-power spectrum beyond linear scales. We make all our measured power spectra public in \url{https://github.com/andreufont/sherwood_p3d}. This study is a step towards joint analyses of 1D and 3D flux correlations, and towards using the quasar-Ly$\alpha$ cross-correlation beyond BAO analyses.

==> other_plots.tex <==
\section{Other plots (to be most likely dropped)}
\label{app:other}

\AFR{I have moved here material from the main text that most likely will not make it to the final paper, at least not in the current form.}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \includegraphics[width=\textwidth]{cross_arinyo_9_9.5_residuals.png}
    \caption[Network2]%
        {{\small Network 1}}      
    \label{fig:mean and std of net14}
    \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{cross_arinyo_9.5_10.5_residuals.png}
            \caption[]%
            {Network 2}    
            \label{fig:mean and std of net24}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{cross_arinyo_10.5_11.5_residuals.png}
            \caption[]%
            {Network 3}    
            \label{fig:mean and std of net34}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{cross_arinyo_11.5_14_residuals.png}
            \caption[]%
            {Network 4}    
            \label{fig:mean and std of net44}
        \end{subfigure}
        \caption[ The average and standard deviation of critical parameters ]
        
        \label{fig:mean and std of nets}
\end{figure}

\AFR{Fig \ref{fig:mean and std of nets} are plots by Jahmour that were in the convergence appendix.}

\subsection{Fits to lowest mass bin}
$\chi^2=499$, degrees of freedom=225

\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
bias\_h  & 1.1040735102748118   \\ \hline
bias\_f  & -0.23533257814840597 \\ \hline
beta\_f  & 1.336825983347525    \\ \hline
d1\_q1   & 0.7507476606990217   \\ \hline
d1\_q2   & 0.08596417609285414  \\ \hline
d1\_kvav & 0.7591587334633261   \\ \hline
d1\_av   & 0.3408764919972579   \\ \hline
d1\_bv   & 1.8175329668556448   \\ \hline
d1\_kp   & 13.731668671423575   \\ \hline
sigmav   & 0.4036419370406364   \\ \hline
gamma    & 0.9991066220095683   \\ \hline
nu       & 0.13264532447883645  \\ \hline
alpha    & 0.023956621167942442 \\ \hline
chi2     & 499.46958690698574   \\ \hline
dof      & 225                  \\ \hline
\end{tabular}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_cross_z28_9M95_L160_N2048.pdf}
    \label{fig:cross_9_95}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_lya_z28_9M95_L160_N2048.pdf}
    \label{fig:lya_9_95}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_halo_z28_9M95_L160_N2048.pdf}
    \label{fig:halo_9_95}
\end{figure}


\subsection{Fits to second-lowest mass bin}
$\chi^2=308$, degrees of freedom=225

\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
bias\_h  & 1.2495319148598703   \\ \hline
bias\_f  & -0.24103382958396558 \\ \hline
beta\_f  & 1.3408058085948467   \\ \hline
d1\_q1   & 0.5464650551124766   \\ \hline
d1\_q2   & 0.2850188838721437   \\ \hline
d1\_kvav & 0.6322105644491587   \\ \hline
d1\_av   & 0.23740912684745064  \\ \hline
d1\_bv   & 1.8114556146896135   \\ \hline
d1\_kp   & 12.36130155666477    \\ \hline
sigmav   & 0.3088113110408205   \\ \hline
gamma    & 0.9677561485323571   \\ \hline
nu       & 0.13527830726300705  \\ \hline
alpha    & 0.16220599557460913  \\ \hline
chi2     & 307.92289453431476   \\ \hline
dof      & 225                  \\ \hline
\end{tabular}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_cross_z28_95M105_L160_N2048.pdf}
    \label{fig:cross_95_105}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_lya_z28_95M105_L160_N2048.pdf}
    \label{fig:lya_95_105}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_halo_z28_95M105_L160_N2048.pdf}
    \label{fig:halo_95_105}
\end{figure}


\subsection{Fits to second-highest mass bin}
$\chi^2=258$, degrees of freedom=225

\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
bias\_h  & 1.8640425943568562   \\ \hline
bias\_f  & -0.2411062648677455  \\ \hline
beta\_f  & 1.2541410501038932   \\ \hline
d1\_q1   & 0.6011720443733855   \\ \hline
d1\_q2   & 0.1941973637177391   \\ \hline
d1\_kvav & 0.7761217495226463   \\ \hline
d1\_av   & 0.35723610007231293  \\ \hline
d1\_bv   & 1.8382393513224322   \\ \hline
d1\_kp   & 13.481020080264742   \\ \hline
sigmav   & 0.2676712300388744   \\ \hline
gamma    & 0.7420564847398687   \\ \hline
nu       & 0.5812896071510905   \\ \hline
alpha    & -0.23273825156255734 \\ \hline
chi2     & 258.0272010711505    \\ \hline
dof      & 225                  \\ \hline
\end{tabular}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_cross_z28_105M115_L160_N2048.pdf}
    \label{fig:cross_105_115}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_lya_z28_105M115_L160_N2048.pdf}
    \label{fig:lya_105_115}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_halo_z28_105M115_L160_N2048.pdf}
    \label{fig:halo_105_115}
\end{figure}


\subsection{Fits to highest mass bin}
$\chi^2=448$, degrees of freedom=225

\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
bias\_h  & 3.287717405926581    \\ \hline
bias\_f  & -0.24591444111119576 \\ \hline
beta\_f  & 1.2929851553987914   \\ \hline
d1\_q1   & 0.4397041992475731   \\ \hline
d1\_q2   & 0.3456827664416283   \\ \hline
d1\_kvav & 0.5982968204564798   \\ \hline
d1\_av   & 0.22400213625354948  \\ \hline
d1\_bv   & 1.8259667032369098   \\ \hline
d1\_kp   & 12.414300695815125   \\ \hline
sigmav   & 0.23687363152548968  \\ \hline
gamma    & 0.5279680191037549   \\ \hline
nu       & 1.1485947964815648   \\ \hline
alpha    & -0.7510671372438091  \\ \hline
chi2     & 447.7478480729131    \\ \hline
dof      & 225                  \\ \hline
\end{tabular}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_cross_z28_115M14_L160_N2048.pdf}
    \label{fig:cross_115_14}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_lya_z28_115M14_L160_N2048.pdf}
    \label{fig:lya_115_14}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{P_halo_z28_115M14_L160_N2048.pdf}
    \label{fig:halo_115_14}
\end{figure}


==> results.tex <==
\section{Results}
\label{sec:results}
Give fits to different mass bins in each subsection below.

\subsection{\lyaf\ power spectrum fits}

\AFR{This has already been moved to section 4}

\subsection{Halo power spectrum fits}
Here we present fits to Equations \ref{eq:kaiser} and \ref{eq:sco} both with and without Equation \ref{eq:Dh} as a multiplicative correction. All fits shown were done on models with shot noise included, though we subtract shot noise from plots for ease of visualization.

Figure \ref{fig:kaiser_fog} shows that a FoG correction term does not affect fits obtained using the Kaiser model up to $k_\textrm{max}=1 \hMpc$. Similarly, Figure \ref{fig:sco_fog} demonstrates only a minor improvement in fit when adding FoG to the Scoccimarro model. The difference appears small enough to warrant against including a FoG correction in these fits, thereby removing $\sigma_v$ as a free parameter in the model. However, this is only true when considering all halos in the snapshot. We find that a FoG correction becomes important if one wants to fit halos in the lowest mass bin. \JG{Mention how we got k=1 as the largest mode we can trust.}

Since the Scoccimarro model outperforms Kaiser, we fit the former to halos segregated into four mass bins. Those results are shown in Figure \ref{fig:mass_bin_fits_halo}. Best-fit values for $b_h$ and $\sigma_v$ as functions of halo mass are plotted in Figure \ref{fig:halo_biases_vs_M}.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{compare_kaiser_fog.png}
    \caption{Comparison of Kaiser halo model with and without fingers-of-God correction.}
    \label{fig:kaiser_fog}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{compare_sco_fog.png}
    \caption{Comparison of Scoccimarro halo model with and without fingers-of-God correction.}
    \label{fig:sco_fog}
\end{figure}

\begin{figure}
\centering
{
  \includegraphics[width=0.48\textwidth]{compare_sco_fog_9_9.5.png}
}
{
  \includegraphics[width=0.48\textwidth]{compare_sco_fog_9.5_10.5.png}
  }
\hspace{0mm}
{
  \includegraphics[width=0.48\textwidth]{compare_sco_fog_10.5_11.5.png}
  }
{
  \includegraphics[width=0.48\textwidth]{compare_sco_fog_11.5_14.png}
  }
\caption{Fits of the Scoccimarro model to halos in different mass bins.}
\label{fig:mass_bin_fits_halo}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{bias_h_vs_M.pdf}
    \includegraphics[width=0.49\textwidth]{sigma_v_vs_M.pdf}
    \caption{Best-fit halo parameters from the Scoccimarro model as functions of mass.}
    \label{fig:halo_biases_vs_M}
\end{figure}

\subsection{\lya\ $\times$ halo cross-power spectrum fits}

To begin, we first show a comparison of fits obtained from the linear theory model of Equation \ref{eq:linear_cross} in Figure \ref{fig:linear_cross_fit} and the ``naive'' model of Equation \ref{eq:naive_cross_model} in Figure \JG{insert}.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{cross_kaiser_fit.png}
    \caption{Best-fit linear theory model for the cross-power spectrum between halos and the \lyaf. The bias parameters were obtained from a joint 3x2-point fit of the halo and \lya auto power spectra and their cross spectrum as discussed in Section \ref{sec:analysis}.}
    \label{fig:linear_cross_fit}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{cross_naive_fit.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

